Non-trivial action of the Johnson filtration on the homology of configuration spaces

We let the mapping class group $\Gamma_{g,1}$ of a genus $g$ surface $\Sigma_{g,1}$ with one boundary component act on the homology $H_*(F_{n}(\Sigma_{g,1});\mathbb{Q})$ of the $n^{th}$ ordered configuration space of the surface. We prove that the action is non-trivial when restricted to the $(n-1)^{st}$ stage of the Johnson filtration, for all $n\ge 1$ and $g\ge 2$. We deduce an analogous result for closed surfaces.

==> 7-smallcomputations.tex <==
\section{Small computations}
In this section we compute $H_*(F_n(\Sigma_2))$ for $n\le4$ and prove the following proposition
\begin{proposition}
\label{prop:smallcomputations}
The action of $J_2(1)\subset\Gamma_2$ on $H_*(F_n(\Sigma_2))$ is trivial for $n\le4$.
\end{proposition}

